TURL: Table Understanding through Representation Learning

Relational tables on the Web store a vast amount of knowledge. Owing to the wealth of such tables, there has been tremendous progress on a variety of tasks in the area of table understanding. However, existing work generally relies on heavily-engineered task-specific features and model architectures. In this paper, we present TURL, a novel framework that introduces the pre-training/fine-tuning paradigm to relational Web tables. During pre-training, our framework learns deep contextualized representations on relational tables in an unsupervised manner. Its universal model design with pre-trained representations can be applied to a wide range of tasks with minimal task-specific fine-tuning. Specifically, we propose a structure-aware Transformer encoder to model the row-column structure of relational tables, and present a new Masked Entity Recovery (MER) objective for pre-training to capture the semantics and knowledge in large-scale unlabeled data. We systematically evaluate TURL with a benchmark consisting of 6 different tasks for table understanding (e.g., relation extraction, cell filling). We show that TURL generalizes well to all tasks and substantially outperforms existing methods in almost all instances.

==> sections/introduction_old.tex <==
\section{Introduction}
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/table_example.png}
\caption{An example of a relational table extracted from Wikipedia.}
\label{fig:example}
\end{figure}
The Web stores a large amount of knowledge in the form of semi-structured tables. There are several advantages of using tables: the column-and-row structure makes them more suited for storing structured knowledge than unstructured web documents; while the less rigid table schema still makes concept representations less complex in contrast to structured knowledge bases. 
Thanks to their versatility and utility, a large number of tables are being generated and are made available on the web.
Among all kinds of web tables, relational tables (also referred to as entity-attribute tables) are a special class that are considered to be of high quality and have been proven to be valuable in assisting users in the process of gathering and processing information of interest \cite{CafarellaHZWW08,cafarella2008webtables,yakout2012infogather}. Such a table consists of multiple entities as keys, along with multiple attributes stored in columns. 

Each of the relational tables essentially forms a small relational database. However, tables on the web also have several unique characteristics that differ them from traditional tables, i.e., tables in relational databases or spreadsheets. First, most web tables are generated by users ad hoc. Oftentimes there is no explicit schema or other metadata. Second, web tables cover a wide range of open domain knowledge. Figure \ref{fig:example} shows an example of a relational table found on the web

A number of web table collections have been developed over the last two decades. \citet{cafarella2008webtables, CafarellaHZWW08} first introduced the concept of relational tables and reported 154M such tables from a general web crawl in 2008. \citet{lehmberg2016large} used the Common Crawl corpus and extracted 233M web tables which are further classified into three categories: relational, entity, and matrix. \citet{bhagavatula2015tabel} focused on Wikipedia instead, and extracted 1.6M high quality relational tables. These data sets have been widely studied for a variety of purposes, including table interpretation \cite{}, table search \cite{}, table augmentation \cite{}, etc. 
\hs{until here, all the above can be merged into the first paragraph. speed up the pace to tell people what you want to do.. See below:}
However, most prior works on relational tables focused on developing task specific models, where tables are usually represented using simple features. 

\hs{Background scheme:} Semi-structured tables are prevalent on the Web. Among them, relational tables (also referred to as entity-attribute tables) are a special class that stores a large amount of knowledge, usually with key entities as one core column and their attributes as other columns. There have been various collections of such tables \cite{cafarella2008webtables, CafarellaHZWW08, bhagavatula2015tabel, lehmberg2016large} over the past decade. For example, \citet{bhagavatula2015tabel} extracted 1.6M high-quality relational tables from Wikipedia.  \nop{\citet{cafarella2008webtables, CafarellaHZWW08} first introduced the concept of relational tables and reported 154M such tables from a general web crawl in 2008. \citet{lehmberg2016large} used the Common Crawl corpus and extracted 233M web tables which are further classified into three categories: relational, entity, and matrix. \citet{bhagavatula2015tabel} focused on Wikipedia intead, and extracted 1.6M high quality relational tables.} These data have been widely used for various tasks, including table interpretation \cite{}, table search \cite{}, table augmentation \cite{}, etc. 

\hs{Research gap or Motivation for your work:} However, most prior works on relational tables focused on developing task specific models, where tables are usually represented using simple features... Inspired by the recent pretraining-then-finetuning paradigm on text data, where advanced language pre-training models like BERT can be directly applied for various tasks via fine-tuning, we investigate this paradigm on semi-structured tables. 

In particular, we focus on \textit{entity-focused relational tables}, which contain high quality relational knowledge about entities... More specifically, unsupervised representation learning on texts~\cite{} and KBs~\cite{} has gained much attention recently. In contrast, only few works studying representation learning on semi-structured tables have been proposed. \cite{} learns embedding for words and entities in tables using Word2Vec by serializing the table and has shown promising results in some table-oriented tasks. However, embeddings learned by \cite{} cannot generate contextualized representation for table elements. Also, shallow neural models like Word2Vec have limited learning capability which prevents them from learning complex semantic pattern and knowledge information contained in relational tables. In this paper, we study the problem of learning  a \textit{contextualized} representation for semi-structured tables that captures the semantic pattern in table schema as well as the knowledge embedded in table body.


\nop{we propose XXX, a novel table pre-training paradigm that learns representation for different elements of relational tables and benefits various table-driven tasks.}

\al{Can you clarify the reference to BERT style pre-training in this context. Is this referring to masked pre-training tasks?  In my understanding, BERT pre-training is novel because it is estimating the joint probability of phrases by capturing the conditional probabilities of words in both directions left to right and right to left with masked token prediction. Does the bi-directional aspect matter in the table context? And if so, why? } \xd{We can view the masked token prediction in BERT as recover based on the context (unmasked tokens), and the context can be on the left/right side, this is what they call it bi-directional. In table, actually there is no direction. We use the same idea of recover based on the context, here the context is defined by table structure (e.g. for an entity in table cell, the context is its column header, column in the same row/column and table caption)}

\hs{Challenges \& How you would like to solve the problem:} To adopt BERT style pre-training on semi-structured tables, there are two main challenges. (1) \textbf{Structured Table Encoding}: existing language pre-training models take inputs as a sequence of words, while data in relational tables are organized in semi-structured form. (2) \textbf{Heterogeneous Information Integration}: a relational table contains multiple elements including caption, headers and cell values. How to correctly represent each component and integrate them together in pre-training is another challenge.

To address the first challenge, we employ a structure-aware transformer encoder with masked self attention. We build an adjacency matrix based on the column-and-row structure. This adjacency matrix is then used as additional mask for transformer encoder, so that each element can only aggregate information from other structure related elements. For the second challenge, we first encode information of different table components into input embeddings and fuse them together. We then design two separate training objectives: (1) masked language model for table schema; (2) masked entity recovery for relational knowledge.\nop{let the model simultaneously learn the semantic pattern in table schema as well as the knowledge embedded in table body.}

\nop{We conduct experiments on several table-driven tasks, i.e., row population, cell filling and attribute discovery. Experimental results show that the representation learned by our pre-trained model significantly boosts the performance of baseline models in all tasks.}

\hs{To facilitate research in this direction, we present the Table Understanding Evaluation Benchmark (TUEB): a benchmark of 7 diverse table-related tasks..}



The contributions of our paper are summarized as follows:



==> sections/response.tex <==
\section{Response to Reviewer Comments}
\subsection{Response to Meta-Reviewer\#1 R1 and Reviewer\#1 R1}
\noindent\textbf{Discussion of existing datasets}
We want to thank the reviewer for pointing out existing benchmarks and providing a detailed list of references. \nop{We considered some of the mentioned datasets when designing the experiments.} Due to space limitation\nop{ in our submission}{, in the initial submission}, we only briefly discussed the existing datasets for each task and mainly focused on providing a clear description of how we created the benchmark and the characteristics of our dataset. \nop{However, }\nop{Make it more concise: }{In this revision, we have made the following changes:}

\begin{itemize}
    \item We have added a new section in related work (Section 3) to discuss the profile of existing web table related benchmarks and how they compare with our benchmark.
    \item Aside from the added discussion, we have also included new experiments on these existing datasets. Specifically, as mentioned by reviewers, existing benchmarks T2D \cite{lehmberg2016large}, Limaye \cite{LimayeGirija2010AnnotatingAS} and ISWC2019 \cite{jimenez2020semtab} were created for evaluating table-to-KB matching systems.  We have utilized these benchmarks in Sections 6.2 and 6.3.  Please see Response A.2 and A.3 for more details. For table augmentation, few datasets have been released \cite{zhang2017entitables, zhang2019auto} and there exists no widely used benchmark. Thus we evaluated on our testing set, but included methods in \cite{zhang2017entitables,zhang2019auto,Deng2019Table2VecNW} as baselines.
\end{itemize}


%agree that a comprehensive discussion of existing datasets would be helpful and have added that to related work. 

\subsection{Response to Meta-Reviewer\#1 R2 and Reviewer\#1 R2}
\noindent\textbf{Evaluation with existing Wikipedia table dataset}
All datasets included in our benchmark are created from Wikipedia tables. \nop{However, to better understand our model in comparison with existing works on Wikipedia tables, we also include the following experiments in the paper:}{To better understand how our model performs, we have added the following experiments for more direct, head-to-head comparison with existing works on previously established benchmarks, both Wikipedia and non-Wikipedia:}
\begin{itemize}
    \item The WikiGS dataset we used in entity linking task is the benchmark created by Efthymiou et al. \cite{Efthymiou2017MatchingWT} from Wikipedia tables. We choose it over Limaye \cite{LimayeGirija2010AnnotatingAS} because it is more challenging due to its structure, diversity, and size \cite{Efthymiou2017MatchingWT}. It is also used in many other recent works \cite{Chen2018ColNetET, Chen2019LearningSA}, and is the source of Wikipedia tables in ISWC2019 \cite{jimenez2020semtab}. For entity linking, aside from the Wikidata Lookup baseline, we selected two systems T2K \cite{Ritze2015MatchingHT} and Hybrid II \cite{Efthymiou2017MatchingWT} out of the ten baselines in \cite{Efthymiou2017MatchingWT} and included their scores {in the original submission}\nop{paper}.
    \item \nop{In this revision, we}{We} have added two new experiments for column type annotation (Section 6.3). (1) We manually map the types used in existing datasets \cite{Chen2019LearningSA} to the types used in our benchmark and directly evaluate\nop{our models on them to see how} our trained models on them\nop{existing datasets}. (2) We follow the same setting as \cite{Chen2019LearningSA}, and use 250 columns in T2Dv2 as training data {to fine-tune our model}.
\end{itemize}

\subsection{Response to Meta-Reviewer\#1 R3, Reviewer\#1 R3, and Reviewer\#3 W1}
\noindent\textbf{Evaluation with Web tables from different websites}
To better understand how our model performs on tables from websites other than Wikipedia, we have added the following experiments using T2D and T2Dv2 \cite{lehmberg2016large}. T2Dv2 is the second version of the T2D entity-level gold standard\nop{. \nop{A principle} Its major difference from T2D is that T2Dv2 does not only contain positive but also negative examples}{, with the major difference that the latter contains only positive examples, whereas the former also contains negative examples}. Here we use the data and annotations {released by baselines compared in this paper}\nop{released by the corresponding papers}\nop{this is vague when connecting it with the previous sentence. corresponding to what?}:
\begin{itemize}
    \item We have added entity linking results on the T2D corpus used in \cite{Efthymiou2017MatchingWT} (Section 6.2). Same as what we did for the WikiGS corpus, we compare with three baselines Wikidata Lookup, T2K \cite{Ritze2015MatchingHT} and Hybrid II \cite{Efthymiou2017MatchingWT}.
    \item \nop{In the two experiments added for column type annotation (described in Response A.2), we have also included results on the T2Dv2 corpus, \hs{following recent work \cite{XX}}.} We have also included results on the T2Dv2 corpus for the new experiments added for column type annotation. Please see Response A.2 for more information.
\end{itemize}

\subsection{Response to Meta-Reviewer\#1 R4 and Reviewer\#3 W2}
\noindent\textbf{More error analysis}
\begin{itemize}
    \item To help understand the strengths and weaknesses of our method, we have added an error analysis and a case study for the entity linking task (Section 6.2) on the T2D dataset.
\end{itemize}

\subsection{Response to Meta-Reviewer\#1 R5 and Reviewer\#3 W3}
\noindent\textbf{Add baseline for relation extraction}
In this work, we defined the task of relation extraction on Web tables in a similar way to relation extraction in natural language processing \cite{riedel2010modeling} (Section 6.4). It differs from existing works like \cite{Mulwad2010UsingLD,Ritze2015MatchingHT,Zhang2017EffectiveAE} in that: (1) we do not rely on entity linking results of table contents, and this allows the extraction of new knowledge; (2) we form the problem as a classification task where we use a predefined closed set of relations as targets. \nop{This is different from \cite{Mulwad2010UsingLD,Ritze2015MatchingHT,Zhang2017EffectiveAE} where they retrieve relations based on entity linking results and use all relations in the knowledge base as targets.} \nop{However, to}{To} better understand the difference between our work and existing ones\nop{ the two settings}, we have added the following experiment in this revision:
\begin{itemize}
    \item The key idea of \cite{Mulwad2010UsingLD,Ritze2015MatchingHT,Zhang2017EffectiveAE} is to first link all cells to the target KB, and then annotate relations based on majority voting of existing relations between linked entities. {We have added results of a similar entity linking based model (Section 6.4)}\nop{We add results to relation extraction using a similar entity linking based model (Section 6.4)}.
\end{itemize}

\subsection{Response to Reviewer\# 2 W3}
\noindent\textbf{References}
We want to thank the reviewer for pointing out the reference. We have added them along with some other related works (Section 3).

==> tables/table_retrieval.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|l|c|c|}
    \hline
        &MAP & P@1  \\
        \hline
        NeuralNet~\cite{Yan2017ContentBasedTR}&&\\
        Ours& &\\ 
    \hline
    \end{tabular}
    \caption{Query-based table retrieval result}
    \label{tab:my_label}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{|l|l|c|c|}
    \hline
    \multicolumn{1}{|c|}{Task} & \multicolumn{1}{c|}{Method} & recall & \# tables \\ \hline
    \multirow{2}{*}{Row population} & Baseline &  &  \\ 
     & Ours &  &  \\ \hline
     \multirow{2}{*}{Cell filling} & Baseline &  &  \\ 
     & Ours &  &  \\ \hline
     \multirow{2}{*}{Schema augmentation} & Baseline &  &  \\ 
     & Ours &  &  \\ \hline
    \end{tabular}
    \caption{Table-based table retrieval result}
    \label{tab:my_label}
\end{table}

==> tables/task_overview.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{|>{\centering\arraybackslash} m{2cm}|>{\centering\arraybackslash} m{2cm}|c|>{\centering\arraybackslash} m{10cm}|}
\hline
\multicolumn{2}{|c|}{Task} & \multicolumn{1}{c|}{Baselines} & \multicolumn{1}{c|}{Finetune Strategy} \\ \hline
 & Entity Linking &\cite{Efthymiou2017MatchingWT,Ritze2015MatchingHT}  & \includegraphics[width=\linewidth]{figures/finetune_EL.png} \\ \cline{2-4} 
 Table Interpretation& Column Type Annotation & \cite{Hulsebos2019SherlockAD} &\vspace{2pt}\includegraphics[width=\linewidth]{figures/finetune_CT.png}  \\ \cline{2-4} 
 & Relation Extraction & \cite{zhang2019ernie} &\vspace{2pt}\includegraphics[width=\linewidth]{figures/finetune_RE.png}  \\ \hline
  & Row Population & \cite{zhang2017entitables, Deng2019Table2VecNW} & \includegraphics[width=0.8\linewidth]{figures/finetune_RP.png} \\ \cline{2-4} 
 \makecell{Table\\Augmentation}& Cell Filling & \cite{zhang2019auto,Deng2019Table2VecNW} &\vspace{2pt}\includegraphics[width=\linewidth]{figures/finetune_CF.png}  \\ \cline{2-4} 
 & Schema Augmentation & \cite{zhang2017entitables} &\vspace{2pt}\includegraphics[width=0.5\linewidth]{figures/finetune_SA.png}  \\ \hline
\end{tabular}
\caption{An overview of our benchmark tasks, baselines, and strategies to fine-tune \modelnospace.}
\vspace{-10pt}
\label{tab:task_overview}
\end{table*}
